DiffIR2VR-Zero: Zero-Shot Video Restoration with Diffusion-based Image Restoration Models

We present DiffIR2VR-Zero, a zero-shot framework that enables any pre-trained image restoration diffusion model to perform high-quality video restoration without additional training. While image diffusion models have shown remarkable restoration capabilities, their direct application to video leads to temporal inconsistencies, and existing video restoration methods require extensive retraining for different degradation types. Our approach addresses these challenges through two key innovations: a hierarchical latent warping strategy that maintains consistency across both keyframes and local frames, and a hybrid token merging mechanism that adaptively combines optical flow and feature matching. Through extensive experiments, we demonstrate that our method not only maintains the high-quality restoration of base diffusion models but also achieves superior temporal consistency across diverse datasets and degradation conditions, including challenging scenarios like 8$\times$ super-resolution and severe noise. Importantly, our framework works with any image restoration diffusion model, providing a versatile solution for video enhancement without task-specific training or modifications. Project page: https://jimmycv07.github.io/DiffIR2VR_web/

==> figs/ablation.tex <==
\begin{figure}[t]
\centering
\resizebox{1.0\columnwidth}{!} 
{
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=\textwidth]{figures/ablation.pdf}
}
% \vspace{-5mm}
\caption{\textbf{Visual ablation of the spatial-aware and padding removal}
\textcolor{magenta} {Figure to be updated}
Correspondences are improved after weighted with spatial distance and padding removal. }
% \vspace{-1mm}
\label{fig:ablation}
\end{figure}

==> figs/correspondence.tex <==
\begin{figure}[t]
\centering
\resizebox{1.0\columnwidth}{!} 
{
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=\textwidth]{figures/correspodence.pdf}
}
% \vspace{-5mm}
\caption{\textbf{Token correspondences identified by flow and cosine similarity.}
Correspondences found by cosine similarity are marked in \textcolor{red}{red}, and found by optical flow are marked in \textcolor{green}{green}.
(\(Top\)) At the beginning of the denoising process, the latents in the UNet downblocks are too noisy for cosine similarity to be effective, making optical flow a more reliable method for identifying matching tokens.
(\(Bottom\)) Flow and cosine similarity often identify different correspondences, so a hybrid approach is more effective by utilizing guidance from both methods.
}
% \vspace{-1mm}
\label{fig:correspondence}
\end{figure}

==> figs/correspondence_pad.tex <==
\begin{figure}[h]
\centering
\resizebox{1.0\columnwidth}{!} 
{
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=\textwidth]{figures/correspondence_pad.pdf}
}
% \vspace{-5mm}
% \caption{\textbf{Token correspondences identified by flow and cosine similarity.}
% Correspondences found by cosine similarity are marked in \textcolor{red}{red}, and found by optical flow are marked in \textcolor{green}{green}.
% (\(Top\)) At the beginning of the denoising process, the latents in the UNet downblocks are too noisy for cosine similarity to be effective, making optical flow a more reliable method for identifying matching tokens.
% (\(Bottom\)) Flow and cosine similarity often identify different correspondences, so a hybrid approach is more effective by utilizing guidance from both methods.
% }
% \vspace{-1mm}
\caption{\textbf{The padded regions affect the matching severely.}}
\label{fig:correspondence_pad_fig}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> tables/SR-Denoise.tex <==
\begin{table*}[t]
\caption{\textbf{Quantitative comparisons of video super-resolution on the DAVIS~\citep{perazzi2016benchmark}, Vid4~\citep{liu2013bayesian} and REDS4~\citep{nah2019ntire} datasets.} The best and second performances are marked in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively. $E_{\text{warp}}^*$ denotes $E_{\text{warp}} (\times 10^{-3})$ and  $E_{\text{inter}}$,
LPIPS$_{\text{inter}}$ denotes interpolation error and LPIPS. - indicates out-of-memory.}
\label{tab:SR}
\vspace{-3mm}
\centering
\resizebox{\textwidth}{!}
{
\begin{tabular}{l|r|rrrrrrrrr}
\toprule 
& & & & & & \multicolumn{2}{c}{SD $\times$4~\cite{sdx4}} & \multicolumn{2}{c}{DiffBIR~\cite{lin2024diffbir}}\\\cmidrule(lr){7-8}\cmidrule(lr){9-10}
& Metrics & BasicVSR++~\cite{chan2022basicvsr++} & RVRT~\cite{liang2022recurrent} & VidToMe~\cite{li2024vidtome} & FMA-Net~\cite{youk2024fmanet} & Frame & {{Ours}} & {Frame} & {{Ours}} \\
\midrule
% \multirow{6}{*}{\rotatebox{90}{SPMCS}} & PSNR $\uparrow$ & 20.913 & \textcolor{red}{21.910} & 20.573 & 20.636 & 21.534 & \textcolor{blue}{21.843} \\
%  & SSIM $\uparrow$ & 0.583  & \textcolor{red}{0.617} & 0.490  & 0.517  & 0.544  & \textcolor{blue}{0.572} \\
%  & LPIPS $\downarrow$ & 0.239  & \textcolor{red}{0.230} & 0.298  & 0.286  & 0.261  & \textcolor{blue}{0.258} \\
%  & $E_{\text{warp}}^* \downarrow$ & 0.135  & \textcolor{red}{0.157} & 1.058  & 8.290  & \textcolor{blue}{0.571}  & \textcolor{blue}{0.571} \\
%  & $E_{\text{inter}} \downarrow$ & 2.008 & \textcolor{red}{3.271} & 13.817 & 11.961 & 10.257 & \textcolor{blue}{9.712} \\
%  & LPIPS$_{\text{inter}}\downarrow$ & 0.005  & \textcolor{red}{0.015} & 0.241  & 0.226  & 0.177  & \textcolor{blue}{0.158} \\
% \midrule
\multirow{6}{*}{\rotatebox{90}{DAVIS $\times$4}} & PSNR $\uparrow$ & 26.576 & 26.595 & 23.014 & \textcolor{red}{25.215} & 23.504 & 23.843 {\small\textbf{(+0.339)}} & 23.780 & \textcolor{blue}{24.182} {\small\textbf{(+0.402)}} \\
 & SSIM $\uparrow$ & 0.743 & 0.744 & 0.566  & \textcolor{red}{0.727} & 0.584  & 0.618 {\small\textbf{(+0.034)}} & 0.601  & \textcolor{blue}{0.621} {\small\textbf{(+0.020)}} \\
 & LPIPS $\downarrow$ & 0.383 & 0.388 & 0.405 & 0.347  & 0.277  & 0.272 {\small\textbf{(-0.005)}} & \textcolor{blue}{0.264} & \textcolor{red}{0.262} {\small\textbf{(-0.002)}} \\
 & $E_{\text{warp}}^* \downarrow$ & 0.090 & 0.090 & 0.520  & \textcolor{red}{0.186} & 0.912  & 0.745 {\small\textbf{(-0.167)}} & {0.654} & \textcolor{blue}{0.474} {\small\textbf{(-0.180)}} \\
 & $E_{\text{inter}} \downarrow$ & 9.115 & 9.135 & \textcolor{blue}{13.676} & \textcolor{red}{11.558} & 18.125 & 17.431 {\small\textbf{(-0.694)}} & 16.529 & 14.666 {\small\textbf{(-1.863)}} \\
 & LPIPS$_{\text{inter}}\downarrow$ & 0.058 & 0.058 & 0.329  & \textcolor{red}{0.078} & 0.292  & 0.274 {\small\textbf{(-0.018)}} & 0.266  & \textcolor{blue}0.232 {\small\textbf{(-0.034)}} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{DAVIS $\times$8}} & PSNR $\uparrow$ & 24.301 & 24.504 & 22.097 & \textcolor{red}{22.690} & 20.268 & 20.519 {\small\textbf{(+0.251)}} & 21.964 & \textcolor{blue}{22.331} {\small\textbf{(+0.367)}} \\
 & SSIM $\uparrow$ & 0.631 & 0.638 & 0.513 & \textcolor{red}{0.594} & 0.446  & 0.424 {\small(-0.022)} & 0.502  & \textcolor{blue}{0.519} {\small\textbf{(+0.017)}} \\
 & LPIPS $\downarrow$ & 0.518 & 0.560 & 0.554  & 0.528  & 0.470  & 0.434 {\small\textbf{(-0.036)}} & \textcolor{red}{0.362} & \textcolor{blue}{0.367} {\small(+0.005)} \\
 & $E_{\text{warp}}^* \downarrow$ & 0.132 & 0.127 & \textcolor{blue}{0.440}  & \textcolor{red}{0.351} & 2.199  & 1.759 {\small\textbf{(-0.440)}} & 0.964 & 0.699 {\small\textbf{(-0.265)}} \\
 & $E_{\text{inter}} \downarrow$ & 9.882 & 9.725 & \textcolor{red}{12.624} & \textcolor{blue}{13.978} & 24.496 & 21.746 {\small\textbf{(-2.750)}} & 17.981 & 15.853 {\small\textbf{(-2.128)}} \\
 & LPIPS$_{\text{inter}}\downarrow$ & 0.088 & 0.081 & 0.388  & \textcolor{red}{0.132} & 0.457  & 0.442 {\small\textbf{(-0.015)}} & 0.372  & \textcolor{blue}{0.333} {\small\textbf{(-0.039)}} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{REDS4 $\times$4}} & PSNR $\uparrow$ & 27.227 & 27.244 & 23.134 & \textcolor{red}{25.829} & 24.189 & 24.226 {\small\textbf{(+0.037)}} & 24.679 & \textcolor{blue}{25.118} {\small\textbf{(+0.439)}} \\
 & SSIM $\uparrow$ & 0.781 & 0.781 & 0.589 & \textcolor{red}{0.761} & 0.638 & 0.641 {\small\textbf{(+0.003)}} & 0.657 & \textcolor{blue}{0.683} {\small\textbf{(+0.026)}} \\
 & LPIPS $\downarrow$ & 0.369 & 0.374 & 0.357 & 0.327 & 0.247 & 0.242 {\small\textbf{(-0.005)}} & \textcolor{red}{0.211} & \textcolor{blue}{0.222} {\small{(+0.011)}} \\
 & $E_{\text{warp}}^* \downarrow$ & 0.134 & 0.133 & 0.579 & \textcolor{red}{0.392} & 0.817 & 0.811 {\small\textbf{(-0.006)}} & 0.704 & \textcolor{blue}{0.499} {\small\textbf{(-0.205)}} \\
 & $E_{\text{inter}} \downarrow$ & 15.799 & 15.838 & \textcolor{red}{17.869} & \textcolor{blue}{19.014} & 22.906 & 22.889 {\small\textbf{(-0.017)}} & 22.305 & 20.130 {\small\textbf{(-2.175)}} \\
 & LPIPS$_{\text{inter}}\downarrow$ & 0.106 & 0.101 & 0.356 & \textcolor{red}{0.133} & 0.295 & 0.281 {\small\textbf{(-0.014)}} & 0.271 & \textcolor{blue}{0.221} {\small\textbf{(-0.050)}} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{REDS4 $\times$8}} & PSNR $\uparrow$ & & & 21.894 & \textcolor{blue}{22.842} & - & - & 22.479 & \textcolor{red}{22.961} {\small\textbf{(+0.482)}} \\
 & SSIM $\uparrow$ & & & 0.532 & \textcolor{red}{0.644} & - & - & 0.559 & \textcolor{blue}{0.590} {\small\textbf{(+0.031)}} \\
 & LPIPS $\downarrow$ & & & 0.538 & 0.423 & - & - & \textcolor{blue}{0.311} & \textcolor{red}{0.306} {\small\textbf{(-0.005)}} \\
 & $E_{\text{warp}}^* \downarrow$ & & & \textcolor{red}{0.423} & 0.753 & - & - & 0.828 & \textcolor{blue}{0.551} {\small\textbf{(-0.277)}} \\
 & $E_{\text{inter}} \downarrow$ & & & \textcolor{red}{15.502} & 21.519 & - & - & 21.76 & \textcolor{blue}{19.382} {\small\textbf{(-2.378)}} \\
 & LPIPS$_{\text{inter}}\downarrow$ & & & 0.412 & \textcolor{red}{0.159} & - & - & 0.351 & \textcolor{blue}{0.287} {\small\textbf{(-0.064)}} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{REDS4 $\times$16}} & PSNR $\uparrow$ & 23.579 & 23.715 & 20.520 & \textcolor{red}{21.569} & 18.706 & 18.858 {\small\textbf{(+0.152)}} & 20.124 & \textcolor{blue}{20.712} {\small\textbf{(+0.588)}} \\
 & SSIM $\uparrow$ & 0.616 & 0.621 & 0.483 & \textcolor{red}{0.570} & 0.461 & 0.410 {\small{(-0.051)}} & 0.461 & \textcolor{blue}{0.509} {\small\textbf{(+0.048)}} \\
 & LPIPS $\downarrow$ & 0.600 & 0.596 & 0.697 & 0.565 & 0.612 & 0.562 {\small\textbf{(-0.050)}} & \textcolor{blue}{0.446} & \textcolor{red}{0.438} {\small\textbf{(-0.008)}} \\
 & $E_{\text{warp}}^* \downarrow$ & 0.084 & 0.085 & \textcolor{red}{0.296} & \textcolor{blue}{0.619} & 2.664 & 2.030 {\small\textbf{(-0.634)}} & 1.168 & 0.665 {\small\textbf{(-0.503)}} \\
 & $E_{\text{inter}} \downarrow$ & 14.069 & 14.267 & \textcolor{red}{12.945} & 18.758 & 28.478 & 24.000 {\small\textbf{(-4.478)}} & 21.33 & \textcolor{blue}{17.731} {\small\textbf{(-3.599)}} \\
 & LPIPS$_{\text{inter}}\downarrow$ & 0.088 & 0.088 & 0.417 & \textcolor{red}{0.139} & 0.559 & 0.493 {\small\textbf{(-0.066)}} & 0.444 & \textcolor{blue}{0.358} {\small\textbf{(-0.086)}} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{Vid4 $\times$4}} & PSNR $\uparrow$ & & & 19.622 & \textcolor{red}{23.209} & 20.047 & 20.134 {\small\textbf{(+0.087)}} & 20.687 & \textcolor{blue}{21.226} {\small\textbf{(+0.539)}} \\
 & SSIM $\uparrow$ & & & 0.425 & \textcolor{red}{0.679} & 0.478 & 0.473 {\small{(-0.005)}} & 0.497 & \textcolor{blue}{0.525} {\small\textbf{(+0.028)}} \\
 & LPIPS $\downarrow$ & & & 0.491 & 0.375 & 0.343 & 0.331 {\small\textbf{(-0.012)}} & \textcolor{blue}{0.329} & \textcolor{red}{0.326} {\small\textbf{(-0.003)}} \\
 & $E_{\text{warp}}^* \downarrow$ & & & 0.687 & \textcolor{red}{0.203} & 1.502 & 1.397 {\small\textbf{(-0.105)}} & 1.156 & \textcolor{blue}{0.677} {\small\textbf{(-0.479)}} \\
 & $E_{\text{inter}} \downarrow$ & & & 11.754 & \textcolor{red}{4.442} & 17.234 & 16.921 {\small\textbf{(-0.313)}} & 15.478 & \textcolor{blue}{11.316} {\small\textbf{(-4.162)}} \\
 & LPIPS$_{\text{inter}}\downarrow$ & & & 0.337 & \textcolor{red}{0.026} & 0.275 & 0.271 {\small\textbf{(-0.004)}} & 0.265 & \textcolor{blue}{0.198} {\small\textbf{(-0.067)}} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{Vid4 $\times$8}} & PSNR $\uparrow$ & & & 18.811 & \textcolor{red}{21.033} & 17.813 & 17.992 {\small\textbf{(+0.179)}} & 18.636 & \textcolor{blue}{19.304} {\small\textbf{(+0.668)}} \\
 & SSIM $\uparrow$ & & & 0.372 & \textcolor{red}{0.521} & 0.345 & 0.307 {\small{(-0.038)}} & 0.367 & \textcolor{blue}{0.406} {\small\textbf{(+0.039)}} \\
 & LPIPS $\downarrow$ & & & 0.654 & 0.514 & 0.507 & 0.484 {\small\textbf{(-0.023)}} & \textcolor{blue}{0.440} & \textcolor{red}{0.435} {\small\textbf{(-0.005)}} \\
 & $E_{\text{warp}}^* \downarrow$ & & & \textcolor{blue}{0.477} & \textcolor{red}{0.221} & 2.523 & 1.972 {\small\textbf{(-0.551)}} & 1.524 & 0.767 {\small\textbf{(-0.757)}} \\
 & $E_{\text{inter}} \downarrow$ & & & \textcolor{blue}{9.942} & \textcolor{red}{5.269} & 22.881 & 19.970 {\small\textbf{(-2.911)}} & 18.112 & 12.281 {\small\textbf{(-5.831)}} \\
 & LPIPS$_{\text{inter}}\downarrow$ & & & 0.393 & \textcolor{red}{0.032} & 0.423 & 0.419 {\small\textbf{(-0.004)}} & 0.395 & \textcolor{blue}{0.294} {\small\textbf{(-0.101)}} \\
\bottomrule
\end{tabular}
}
\end{table*}












\begin{table}[t]
\caption{\textbf{Quantitative comparisons of video denoising of various noise levels on the REDS30 and Set8~\citep{Set8} dataset.} The best and second performances are marked in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively. $E_{\text{warp}}^*$ denotes $E_{\text{warp}} (\times 10^{-3})$ and  $E_{\text{inter}}$,
LPIPS$_{\text{inter}}$ denotes interpolation error and LPIPS.}
\label{tab:denoise}
\centering
\resizebox{\columnwidth}{!}
{
\begin{tabular}{c|r|rrrr}
\toprule
& & & & \multicolumn{2}{c}{DiffBIR~\cite{lin2024diffbir}}\\\cmidrule(lr){5-6}
 $\sigma$ & Metrics  & {VidToMe~\cite{li2024vidtome}} & {Shift-Net~\cite{yan2018shift}} & {Frame} & {Ours} \\
\midrule
 \multirow{6}{*}{\rotatebox{90}{REDS30 75}} & PSNR $\uparrow$ & 22.671 & 21.033 & \textcolor{red}{24.585} & \textcolor{blue}{24.520} \\
 & SSIM $\uparrow$ & 0.559  & 0.381  & \textcolor{red}{0.649} & \textcolor{red}{0.649}  \\
 & LPIPS $\downarrow$ & 0.397  & 0.735  & \textcolor{blue}{0.276} & \textcolor{red}{0.275}  \\
 & $E_{\text{warp}}^* \downarrow$ & \textcolor{blue}{0.727} & 0.765  & 0.751 & \textcolor{red}{0.706}  \\
 & $E_{\text{inter}} \downarrow$ & \textcolor{red}{18.440} & 21.751 & 21.798 & \textcolor{blue}{21.166} \\
 & LPIPS$_{\text{inter}}\downarrow$ & 0.375  & 0.501  & \textcolor{red}{0.275} & \textcolor{red}{0.264}  \\\midrule
 \multirow{6}{*}{\rotatebox{90}{REDS30 100}} & PSNR $\uparrow$ & 22.588 & 22.573 & \textcolor{blue}{24.524} & \textcolor{red}{24.534} \\
 & SSIM $\uparrow$ & 0.557  & 0.484   & \textcolor{blue}{0.648} & \textcolor{red}{0.652}  \\
 & LPIPS $\downarrow$ & 0.404  & 0.518 & \textcolor{blue}{0.275} & \textcolor{red}{0.271}  \\
& $E_{\text{warp}}^* \downarrow$ & \textcolor{blue}{0.733}  & 1.126 & 0.763 & \textcolor{red}{0.696}  \\
& $E_{\text{inter}} \downarrow$ & \textcolor{red}{18.370} & 23.424 & 21.835 & \textcolor{red}{20.639} \\
& LPIPS$_{\text{inter}}\downarrow$ & 0.380  & 0.375 & \textcolor{blue}{0.281} & \textcolor{red}{0.267}  \\ \midrule
\multirow{6}{*}{\rotatebox{90}{REDS30 random}} & PSNR $\uparrow$ & 22.348 & 21.113 & \textcolor{red}{24.579} & \textcolor{blue}{24.508} \\
& SSIM $\uparrow$ & 0.546  & 0.386 & \textcolor{red}{0.650} & \textcolor{blue}{0.649}  \\
& LPIPS $\downarrow$ & 0.429 & 0.728 & \textcolor{blue}{0.276} & \textcolor{red}{0.270}  \\
& $E_{\text{warp}}^* \downarrow$ & \textcolor{red}{0.681} & 1.896 & 0.755 & \textcolor{blue}{0.713}  \\
& $E_{\text{inter}} \downarrow$ & \textcolor{red}{17.608} & 27.565 & 21.743 & \textcolor{blue}{21.140} \\
& LPIPS$_{\text{inter}}\downarrow$ & 0.384  & 0.542 & \textcolor{blue}{0.282} & \textcolor{red}{0.272}  \\ \midrule
\multirow{6}{*}{\rotatebox{90}{Set8 50}} & PSNR $\uparrow$ & 21.531 & \textcolor{blue}{23.433} & 23.197 & \textcolor{red}{23.713} \\
& SSIM $\uparrow$ & 0.501 & 0.482 & \textcolor{blue}{0.594} & \textcolor{red}{0.63} \\
& LPIPS $\downarrow$ & 0.415 & 0.574 & \textcolor{blue}{0.261} & \textcolor{red}{0.245} \\
& $E_{\text{warp}}^* \downarrow$ & \textcolor{blue}{0.911} & 1.358 & 1.078 & \textcolor{red}{0.747} \\
& $E_{\text{inter}} \downarrow$ & \textcolor{blue}{17.217} & 19.845 & 19.732 & \textcolor{red}{16.814} \\
& LPIPS$_{\text{inter}}\downarrow$ & 0.406 & 0.432 & \textcolor{blue}{0.332} & \textcolor{red}{0.255} \\ \midrule
\multirow{6}{*}{\rotatebox{90}{Set8 100}} & PSNR $\uparrow$ & 21.226 & 18.198 & \textcolor{blue}{22.519} & \textcolor{red}{22.955} \\
& SSIM $\uparrow$ & 0.484 & 0.281 & \textcolor{blue}{0.553} & \textcolor{red}{0.591} \\
& LPIPS $\downarrow$ & 0.472 & 0.733 & \textcolor{blue}{0.338} & \textcolor{red}{0.323} \\
& $E_{\text{warp}}^* \downarrow$ & \textcolor{blue}{0.918} & 2.229 & 1.13 & \textcolor{red}{0.802} \\
& $E_{\text{inter}} \downarrow$ & \textcolor{red}{17.367} & 24.661 & 20.18 & \textcolor{blue}{17.444} \\
& LPIPS$_{\text{inter}}\downarrow$ & 0.421 & 0.619 & \textcolor{blue}{0.372} & \textcolor{red}{0.286} \\ \midrule
\multirow{6}{*}{\rotatebox{90}{Set8 150}} & PSNR $\uparrow$ & 20.209 & 16.136 & \textcolor{blue}{21.005} & \textcolor{red}{21.418} \\
& SSIM $\uparrow$ & 0.443 & 0.291 & \textcolor{blue}{0.486} & \textcolor{red}{0.544} \\
& LPIPS $\downarrow$ & 0.554 & 0.729 & \textcolor{blue}{0.449} & \textcolor{red}{0.402} \\
& $E_{\text{warp}}^* \downarrow$ & \textcolor{blue}{0.972} & 4.279 & 1.207 & \textcolor{red}{0.832} \\
& $E_{\text{inter}} \downarrow$ & \textcolor{blue}{17.872} & 22.343 & 20.729 & \textcolor{red}{17.616} \\
& LPIPS$_{\text{inter}}\downarrow$ & 0.470 & 0.646 & \textcolor{blue}{0.450} & \textcolor{red}{0.331} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/SR-Denoise_new.tex <==
\begin{table}[t]
\caption{\textbf{Quantitative comparisons.} (\emph{Left}) Video super-resolution on the DAVIS~\citep{perazzi2016benchmark}, Vid4~\citep{liu2013bayesian} and REDS4~\citep{nah2019ntire} datasets. (\emph{Right}) video denoising of various noise levels on the REDS30 and Set8~\citep{Set8} dataset. The best and second performances are marked in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively. $E_{\text{warp}}^*$ denotes $E_{\text{warp}} (\times 10^{-3})$ and  $E_{\text{inter}}$,
LPIPS$_{\text{inter}}$ denotes interpolation error and LPIPS. - indicates out-of-memory.}
\vspace{-3mm}
\begin{minipage}{.527\linewidth}
\centering
\resizebox{\textwidth}{!}
{
\begin{tabular}{l|r|rrrrrrr}
\toprule 
& & & & \multicolumn{2}{c}{SD $\times$4} & \multicolumn{2}{c}{DiffBIR}\\\cmidrule(lr){5-6}\cmidrule(lr){7-8}
& Metrics & {VidToMe} & {FMA-Net} & Frame & {{Ours}} & {Frame} & {{Ours}} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{DAVIS $\times$4}} & PSNR $\uparrow$ & 23.014 & \textcolor{red}{25.215} & 23.504 & 23.843 & 23.780 & \textcolor{blue}{24.182} \\
 & SSIM $\uparrow$ & 0.566  & \textcolor{red}{0.727} & 0.584  & 0.618 & 0.601  & \textcolor{blue}{0.621} \\
 & LPIPS $\downarrow$ & 0.405 & 0.347  & 0.277  & 0.272 & \textcolor{blue}{0.264} & \textcolor{red}{0.262} \\
 & $E_{\text{warp}}^* \downarrow$ & 0.520  & \textcolor{red}{0.186} & 0.912  & 0.745 & {0.654} & \textcolor{blue}{0.474} \\
 & $E_{\text{inter}} \downarrow$ & \textcolor{blue}{13.676} & \textcolor{red}{11.558} & 18.125 & 17.431 & 16.529 & 14.666 \\
 & LPIPS$_{\text{inter}}\downarrow$ & 0.329  & \textcolor{red}{0.078} & 0.292  & 0.274 & 0.266  & \textcolor{blue}0.232 \\
\midrule
\multirow{6}{*}{\rotatebox{90}{DAVIS $\times$8}} & PSNR $\uparrow$ & 22.097 & \textcolor{red}{22.690} & 20.268 & 20.519 & 21.964 & \textcolor{blue}{22.331} \\
 & SSIM $\uparrow$ & 0.513 & \textcolor{red}{0.594} & 0.446  & 0.424 & 0.502  & \textcolor{blue}{0.519} \\
 & LPIPS $\downarrow$ & 0.554  & 0.528  & 0.470  & 0.434 & \textcolor{red}{0.362} & \textcolor{blue}{0.367} \\
 & $E_{\text{warp}}^* \downarrow$ & \textcolor{blue}{0.440}  & \textcolor{red}{0.351} & 2.199  & 1.759 & 0.964 & 0.699 \\
 & $E_{\text{inter}} \downarrow$ & \textcolor{red}{12.624} & \textcolor{blue}{13.978} & 24.496 & 21.746 & 17.981 & 15.853 \\
 & LPIPS$_{\text{inter}}\downarrow$ & 0.388  & \textcolor{red}{0.132} & 0.457  & 0.442 & 0.372  & \textcolor{blue}{0.333} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{REDS4 $\times$4}} & PSNR $\uparrow$ & 23.134 & \textcolor{red}{25.829} & 24.189 & 24.226 & 24.679 & \textcolor{blue}{25.118} \\
 & SSIM $\uparrow$ & 0.589 & \textcolor{red}{0.761} & 0.638 & 0.641 & 0.657 & \textcolor{blue}{0.683} \\
 & LPIPS $\downarrow$ & 0.357 & 0.327 & 0.247 & 0.242 & \textcolor{red}{0.211} & \textcolor{blue}{0.222} \\
 & $E_{\text{warp}}^* \downarrow$ & 0.579 & \textcolor{red}{0.392} & 0.817 & 0.811 & 0.704 & \textcolor{blue}{0.499} \\
 & $E_{\text{inter}} \downarrow$ & \textcolor{red}{17.869} & \textcolor{blue}{19.014} & 22.906 & 22.889 & 22.305 & 20.130 \\
 & LPIPS$_{\text{inter}}\downarrow$ & 0.356 & \textcolor{red}{0.133} & 0.295 & 0.281 & 0.271 & \textcolor{blue}{0.221} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{REDS4 $\times$8}} & PSNR $\uparrow$ & 21.894 & \textcolor{blue}{22.842} & - & - & 22.479 & \textcolor{red}{22.961} \\
 & SSIM $\uparrow$ & 0.532 & \textcolor{red}{0.644} & - & - & 0.559 & \textcolor{blue}{0.59} \\
 & LPIPS $\downarrow$ & 0.538 & 0.423 & - & - & \textcolor{blue}{0.311} & \textcolor{red}{0.306} \\
 & $E_{\text{warp}}^* \downarrow$ & \textcolor{red}{0.423} & 0.753 & - & - & 0.828 & \textcolor{blue}{0.551} \\
 & $E_{\text{inter}} \downarrow$ & \textcolor{red}{15.502} & 21.519 & - & - & 21.76 & \textcolor{blue}{19.382} \\
 & LPIPS$_{\text{inter}}\downarrow$ & 0.412 & \textcolor{red}{0.159} & - & - & 0.351 & \textcolor{blue}{0.287} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{REDS4 $\times$16}} & PSNR $\uparrow$ & 20.520 & \textcolor{red}{21.569} & 18.706 & 18.858 & 20.124 & \textcolor{blue}{20.712} \\
 & SSIM $\uparrow$ & 0.483 & \textcolor{red}{0.570} & 0.461 & 0.410 & 0.461 & \textcolor{blue}{0.509} \\
 & LPIPS $\downarrow$ & 0.697 & 0.565 & 0.612 & 0.562 & \textcolor{blue}{0.446} & \textcolor{red}{0.438} \\
 & $E_{\text{warp}}^* \downarrow$ & \textcolor{red}{0.296} & \textcolor{blue}{0.619} & 2.664 & 2.030 & 1.168 & 0.665 \\
 & $E_{\text{inter}} \downarrow$ & \textcolor{red}{12.945} & 18.758 & 28.478 & 24.000 & 21.33 & \textcolor{blue}{17.731} \\
 & LPIPS$_{\text{inter}}\downarrow$ & 0.417 & \textcolor{red}{0.139} & 0.559 & 0.493 & 0.444 & \textcolor{blue}{0.358} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{Vid4 $\times$4}} & PSNR $\uparrow$ & 19.622 & \textcolor{red}{23.209} & 20.047 & 20.134 & 20.687 & \textcolor{blue}{21.226} \\
 & SSIM $\uparrow$ & 0.425 & \textcolor{red}{0.679} & 0.478 & 0.473 & 0.497 & \textcolor{blue}{0.525} \\
 & LPIPS $\downarrow$ & 0.491 & 0.375 & 0.343 & 0.331 & \textcolor{blue}{0.329} & \textcolor{red}{0.326} \\
 & $E_{\text{warp}}^* \downarrow$ & 0.687 & \textcolor{red}{0.203} & 1.502 & 1.397 & 1.156 & \textcolor{blue}{0.677} \\
 & $E_{\text{inter}} \downarrow$ & 11.754 & \textcolor{red}{4.442} & 17.234 & 16.921 & 15.478 & \textcolor{blue}{11.316} \\
 & LPIPS$_{\text{inter}}\downarrow$ & 0.337 & \textcolor{red}{0.026} & 0.275 & 0.271 & 0.265 & \textcolor{blue}{0.198} \\
\midrule
\multirow{6}{*}{\rotatebox{90}{Vid4 $\times$8}} & PSNR $\uparrow$ & 18.811 & \textcolor{red}{21.033} & 17.813 & 17.992 & 18.636 & \textcolor{blue}{19.304} \\
 & SSIM $\uparrow$ & 0.372 & \textcolor{red}{0.521} & 0.345 & 0.307 & 0.367 & \textcolor{blue}{0.406} \\
 & LPIPS $\downarrow$ & 0.654 & 0.514 & 0.507 & 0.484 & \textcolor{blue}{0.440} & \textcolor{red}{0.435} \\
 & $E_{\text{warp}}^* \downarrow$ & \textcolor{blue}{0.477} & \textcolor{red}{0.221} & 2.523 & 1.972 & 1.524 & 0.767 \\
 & $E_{\text{inter}} \downarrow$ & \textcolor{blue}{9.942} & \textcolor{red}{5.269} & 22.881 & 19.970 & 18.112 & 12.281 \\
 & LPIPS$_{\text{inter}}\downarrow$ & 0.393 & \textcolor{red}{0.032} & 0.423 & 0.419 & 0.395 & \textcolor{blue}{0.294} \\
\bottomrule
\end{tabular}
}
\label{tab:SR}
\end{minipage}
\hfill
\begin{minipage}{.463\linewidth}
\vspace{-1.5mm}
\centering
\label{tab:denoise}
\resizebox{\textwidth}{!}
{
\begin{tabular}{c|r|rrrr}
\toprule
& & & & \multicolumn{2}{c}{DiffBIR}\\\cmidrule(lr){5-6}
 $\sigma$ & Metrics  & {VidToMe} & {Shift-Net} & {Frame} & {Ours} \\
\midrule
 \multirow{6}{*}{\rotatebox{90}{REDS30 75}} & PSNR $\uparrow$ & 22.671 & 21.033 & \textcolor{red}{24.585} & \textcolor{blue}{24.520} \\
 & SSIM $\uparrow$ & 0.559  & 0.381  & \textcolor{red}{0.649} & \textcolor{red}{0.649}  \\
 & LPIPS $\downarrow$ & 0.397  & 0.735  & \textcolor{blue}{0.276} & \textcolor{red}{0.275}  \\
 & $E_{\text{warp}}^* \downarrow$ & \textcolor{blue}{0.727} & 0.765  & 0.751 & \textcolor{red}{0.706}  \\
 & $E_{\text{inter}} \downarrow$ & \textcolor{red}{18.440} & 21.751 & 21.798 & \textcolor{blue}{21.166} \\
 & LPIPS$_{\text{inter}}\downarrow$ & 0.375  & 0.501  & \textcolor{red}{0.275} & \textcolor{red}{0.264}  \\\midrule
 \multirow{6}{*}{\rotatebox{90}{REDS30 100}} & PSNR $\uparrow$ & 22.588 & 22.573 & \textcolor{blue}{24.524} & \textcolor{red}{24.534} \\
 & SSIM $\uparrow$ & 0.557  & 0.484   & \textcolor{blue}{0.648} & \textcolor{red}{0.652}  \\
 & LPIPS $\downarrow$ & 0.404  & 0.518 & \textcolor{blue}{0.275} & \textcolor{red}{0.271}  \\
& $E_{\text{warp}}^* \downarrow$ & \textcolor{blue}{0.733}  & 1.126 & 0.763 & \textcolor{red}{0.696}  \\
& $E_{\text{inter}} \downarrow$ & \textcolor{red}{18.370} & 23.424 & 21.835 & \textcolor{red}{20.639} \\
& LPIPS$_{\text{inter}}\downarrow$ & 0.380  & 0.375 & \textcolor{blue}{0.281} & \textcolor{red}{0.267}  \\ \midrule
\multirow{6}{*}{\rotatebox{90}{REDS30 random}} & PSNR $\uparrow$ & 22.348 & 21.113 & \textcolor{red}{24.579} & \textcolor{blue}{24.508} \\
& SSIM $\uparrow$ & 0.546  & 0.386 & \textcolor{red}{0.650} & \textcolor{blue}{0.649}  \\
& LPIPS $\downarrow$ & 0.429 & 0.728 & \textcolor{blue}{0.276} & \textcolor{red}{0.270}  \\
& $E_{\text{warp}}^* \downarrow$ & \textcolor{red}{0.681} & 1.896 & 0.755 & \textcolor{blue}{0.713}  \\
& $E_{\text{inter}} \downarrow$ & \textcolor{red}{17.608} & 27.565 & 21.743 & \textcolor{blue}{21.140} \\
& LPIPS$_{\text{inter}}\downarrow$ & 0.384  & 0.542 & \textcolor{blue}{0.282} & \textcolor{red}{0.272}  \\ \midrule
\multirow{6}{*}{\rotatebox{90}{Set8 50}} & PSNR $\uparrow$ & 21.531 & \textcolor{blue}{23.433} & 23.197 & \textcolor{red}{23.713} \\
& SSIM $\uparrow$ & 0.501 & 0.482 & \textcolor{blue}{0.594} & \textcolor{red}{0.63} \\
& LPIPS $\downarrow$ & 0.415 & 0.574 & \textcolor{blue}{0.261} & \textcolor{red}{0.245} \\
& $E_{\text{warp}}^* \downarrow$ & \textcolor{blue}{0.911} & 1.358 & 1.078 & \textcolor{red}{0.747} \\
& $E_{\text{inter}} \downarrow$ & \textcolor{blue}{17.217} & 19.845 & 19.732 & \textcolor{red}{16.814} \\
& LPIPS$_{\text{inter}}\downarrow$ & 0.406 & 0.432 & \textcolor{blue}{0.332} & \textcolor{red}{0.255} \\ \midrule
\multirow{6}{*}{\rotatebox{90}{Set8 100}} & PSNR $\uparrow$ & 21.226 & 18.198 & \textcolor{blue}{22.519} & \textcolor{red}{22.955} \\
& SSIM $\uparrow$ & 0.484 & 0.281 & \textcolor{blue}{0.553} & \textcolor{red}{0.591} \\
& LPIPS $\downarrow$ & 0.472 & 0.733 & \textcolor{blue}{0.338} & \textcolor{red}{0.323} \\
& $E_{\text{warp}}^* \downarrow$ & \textcolor{blue}{0.918} & 2.229 & 1.13 & \textcolor{red}{0.802} \\
& $E_{\text{inter}} \downarrow$ & \textcolor{red}{17.367} & 24.661 & 20.18 & \textcolor{blue}{17.444} \\
& LPIPS$_{\text{inter}}\downarrow$ & 0.421 & 0.619 & \textcolor{blue}{0.372} & \textcolor{red}{0.286} \\ \midrule
\multirow{6}{*}{\rotatebox{90}{Set8 150}} & PSNR $\uparrow$ & 20.209 & 16.136 & \textcolor{blue}{21.005} & \textcolor{red}{21.418} \\
& SSIM $\uparrow$ & 0.443 & 0.291 & \textcolor{blue}{0.486} & \textcolor{red}{0.544} \\
& LPIPS $\downarrow$ & 0.554 & 0.729 & \textcolor{blue}{0.449} & \textcolor{red}{0.402} \\
& $E_{\text{warp}}^* \downarrow$ & \textcolor{blue}{0.972} & 4.279 & 1.207 & \textcolor{red}{0.832} \\
& $E_{\text{inter}} \downarrow$ & \textcolor{blue}{17.872} & 22.343 & 20.729 & \textcolor{red}{17.616} \\
& LPIPS$_{\text{inter}}\downarrow$ & 0.470 & 0.646 & \textcolor{blue}{0.450} & \textcolor{red}{0.331} \\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\end{minipage}
\end{table}


==> tables/ablation1.tex <==
% \begin{table}[h]
% \centering
% \caption{Ablation study of different methods for finding correspondences and their order.}
% % \resizebox{0.65\textwidth}{!}{
% \begin{tabular}{c|cccc}
% \toprule
% Exp.  & PSNR $\uparrow$ & SSIM $\uparrow$ & $E_{\text{warp}}^* \downarrow$& $E_{\text{warp}}^* \downarrow$ \\
% \midrule
% (a) all flow & 23.82 & 0.6385 & 2.398 &\\
% (b) all cosine similarity & 25.47 & 0.7215 & 1.815 &\\
% (c) coisne similarity + flow & 25.75 & \textbf{0.7328} & 0.842 &\\
% (d) flow + coisne similarity (Ours)  & \textbf{25.83} & 0.7326 & \textbf{0.737} &\\
% (e) flow + coisne similarity + spatial-aware (Ours)  & \textbf{25.83} & 0.7326 & \textbf{0.737} &\\
% \bottomrule
% \end{tabular}
% % }
% \label{tab:ablation1}
% \end{table}



% \begin{table}[h]
% \centering
% \caption{\textbf{Ablation study of different correspondence matching methods.}}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{ccccccc|ccc}
% \toprule
% % \multicolumn{2}{c}{Optical flow} & & \multicolumn{2}{c}{Cosine similarity}  \\ \cmidrule{1-2} \cmidrule{4-5}
% % Down blocks & Up blocks & & Down blocks & Up blocks & & Spatial-aware & PSNR $\uparrow$ & SSIM $\uparrow$ & $E_{\text{warp}}^* \downarrow$ \\
% \multicolumn{2}{c}{Down blocks} & & \multicolumn{2}{c}{Up blocks} & & & & & \\ \cmidrule{1-2} \cmidrule{4-5}
% Optical flow & Cosine similarity & & Optical flow & Cosine similarity & & Spatial-aware & PSNR $\uparrow$ & SSIM $\uparrow$ & $E_{\text{warp}}^* \downarrow$ \\
% \midrule
% \checkmark & - & & \checkmark & - & & - & 23.82 & 0.6385 & 2.398 \\
% - & \checkmark & & - & \checkmark & & - & 25.47 & 0.7215 & 1.815 \\
% - & \checkmark & & \checkmark & - & & - & 25.75 & \textbf{0.7328} & 0.842 \\
% \checkmark & - & & - & \checkmark & & - & \textbf{25.83} & 0.7326 & \textbf{0.737} \\
% \checkmark & - & & - & \checkmark & & \checkmark & \textbf{25.83} & 0.7326 & \textbf{0.737} \\
% \bottomrule
% \end{tabular}
% }
% \label{tab:ablation1}
% \end{table}


\begin{table}[tb]
\centering
\caption{\textbf{Ablation study of different correspondence matching methods for 8$\times$ VSR on DAVIS~\cite{7780454}  test sets.}~\yulunliu{Need to explain Flow and Cosine, and refer to the corresponding sections.} \zwc{Also spatial-aware}}
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{llc|ccc}
\toprule
\makecell{Down\\blocks} & \makecell{Up\\blocks} & \makecell{Spatial-\\aware} & LPIPS $\downarrow$ & $E_{\text{warp}}^* \downarrow$  & LPIPS$_{\text{inter}}\downarrow$ \\
\midrule
Flow & Flow & -- & 0.518 & 1.214 & 0.563 \\
Cos & Cos & -- & 0.390 & 0.736 & 0.350 \\
Cos & Flow & -- & 0.507 & 1.049 & 0.545 \\
Flow & Cos & -- & 0.375 & \best{0.677} & 0.347 \\
Flow & Cos & \checkmark &  \best{0.367} & 0.699 & \best{0.333} \\
\bottomrule
\end{tabular}
}
\label{tab:ablation1}
\end{table}

==> tables/ablation2.tex <==
\begin{table}[tb]
\centering
\caption{\textbf{Ablation study of the proposed components applied at different stages of the denoising process.} 
% We apply our two proposed components, hierarchical latent warping (HLW) and hybrid spatial-aware token merging (HS-ToMe) at the early, mid, and late stages of the denoising process.
}
\resizebox{0.6\textwidth}{!}{
\begin{tabular}{ccccccc|ccc}
% \begin{tabular}{*{3}{p{1.5cm}}c*{3}{p{1.5cm}}|ccc}
\toprule
\multicolumn{3}{c}{HLW (Sec.~\ref{subsec:3_3})} & & \multicolumn{3}{c|}{HS-ToMe (Sec.~\ref{subsec:3_4})} \\ \cmidrule{1-3} \cmidrule{5-7}
\centering Early & \centering Mid & \centering Late & & \centering Early & \centering Mid & \centering Late & LPIPS $\downarrow$ & $E_{\text{warp}}^* \downarrow$  & LPIPS$_{\text{inter}}\downarrow$ \\
\midrule
\centering -- & \centering -- & \centering -- & & \centering -- & \centering -- & \centering -- & \textbf{0.362} & 0.964 & 0.372 \\
\centering \checkmark & \centering -- & \centering -- & & \centering \checkmark & \centering -- & \centering -- & 0.368 & 0.887 & 0.369 \\
\centering \checkmark & \centering \checkmark & \centering -- & & \centering \checkmark & \centering \checkmark & \centering \checkmark & 0.43 & 0.804 & 0.183 \\
\centering \checkmark & \centering \checkmark & \centering \checkmark & & \centering \checkmark & \centering \checkmark & \centering \checkmark & 0.411 & 0.704 & 0.339 \\
\centering \checkmark & \centering -- & \centering -- & & \centering \checkmark & \centering \checkmark & \centering \checkmark & 0.367 & \textbf{0.699} & \textbf{0.333} \\
% $\times$ & $\times$ & 23.82 & 0.6385 & 2.398 \\
% initial & initial & 23.82 & 0.6385 & 2.398 \\
% initial \& intermediate & initial & 23.82 & 0.6385 & 2.398 \\
% initial \& intermediate \& final & initial & 23.82 & 0.6385 & 2.398 \\
% initial & initial \& intermediate \& 
% final & 25.47 & 0.7215 & 1.815 \\
\bottomrule
\end{tabular}
}
\label{tab:ablation2}
\end{table}

==> tables/ref.tex <==
\begin{table*}[tb]
\centering
\caption{\textbf{Quantitative results on the LLFF~\cite{mildenhall2019local} dataset.} Our FurgalNeRF performs on par with baseline methods under extreme few-shot settings but with shorter training time and does not rely on any externally learned priors. Most results come from SimpleNeRF~\cite{somraj2023simplenerf}, except VGOS~\cite{sun2023vgos} and SparseNeRF~\cite{wang2023sparsenerf}, for which we run their official implementations with default settings. We mark the best, second-best, and third-best entries in red, orange, and yellow, respectively.}
\vspace{-2mm}
\label{tab:quantitative_llff}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l|c|c|ccc|ccc|ccc|c}
\toprule
 & & Learned & \multicolumn{3}{c|}{2-view} & \multicolumn{3}{c|}{3-view} & \multicolumn{3}{c|}{4-view} & Training \\
Method & Venue & priors & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & time $\downarrow$\\
\midrule
RegNeRF~\cite{niemeyer2022regnerf} & CVPR 2022 & normalizing flow & 16.88 & 0.49 & 0.43 & 18.65 & 0.57 & 0.36 & 19.89 & 0.62 & \cellcolor{yellow!25}0.32 & 2.35 hrs\\
DS-NeRF~\cite{deng2022depth} & CVPR 2022 & - & 16.93 & 0.51 & 0.42 & 18.97 & 0.58 & 0.36 & 20.07 & 0.61 & 0.34 & 3.5 hrs \\
DDP-NeRF~\cite{roessle2022dense} & CVPR 2022 & depth completion & 17.19 & \cellcolor{orange!25}0.54 & 0.39 & 17.71 & 0.56 & 0.39 & 19.19 & 0.61 & 0.35 & 3.5 hrs \\
FreeNeRF~\cite{yang2023freenerf} & CVPR 2023 & - & 17.55 & \cellcolor{orange!25}0.54 & \cellcolor{yellow!25}0.38 & 19.30 & \cellcolor{yellow!25}0.60 & \cellcolor{yellow!25}0.34 & \cellcolor{yellow!25}20.45 & \cellcolor{yellow!25}0.63 & 0.33 & 1.5 hrs\\
ViP-NeRF~\cite{somraj2023vip} & SIGGRAPH 2023 & - & 16.66 & \cellcolor{yellow!25}0.52 & \cellcolor{orange!25}0.37 & 18.89 & 0.59 & \cellcolor{yellow!25}0.34 & 19.34 & 0.62 & \cellcolor{yellow!25}0.32 & 13.5 hrs \\
SimpleNeRF~\cite{somraj2023simplenerf} & SIGGRAPH Asia 2023 & - & \cellcolor{yellow!25}17.57 & \cellcolor{red!25}0.55 & 0.39 & \cellcolor{orange!25}19.47 & \cellcolor{red!25}0.62 & \cellcolor{orange!25}0.33 & 20.44 & \cellcolor{red!25}0.65 & \cellcolor{orange!25}0.31&9.5 hrs \\
VGOS~\cite{sun2023vgos} & IJCAI 2023 & - & 16.75 & \cellcolor{red!25}0.55 & 0.42 & 18.80 & \cellcolor{orange!25}0.61 & 0.37 & 19.69 & \cellcolor{orange!25}0.64 & 0.37&\cellcolor{red!25} 5 mins\\ 
SparseNeRF~\cite{wang2023sparsenerf} & ICCV 2023 & monocular depth  &  \cellcolor{orange!25}18.02 & \cellcolor{yellow!25}0.52 & 0.45 & \cellcolor{red!25}19.52 & 0.59 & 0.37 & \cellcolor{orange!25}20.89 & \cellcolor{red!25}0.65 & 0.34 & \cellcolor{yellow!25}1 hrs \\
FrugalNeRF (Ours) & - & - & \cellcolor{red!25}18.07 & \cellcolor{orange!25}0.54 & \cellcolor{red!25}0.35 & \cellcolor{yellow!25}19.40 & \cellcolor{yellow!25}0.60 & \cellcolor{red!25}0.31 & \cellcolor{red!25}20.95 & \cellcolor{red!25}0.65 & \cellcolor{red!25}0.28 & \cellcolor{orange!25}10 mins\\
 \bottomrule
\end{tabular}%
}
\end{table*}
